Unbiased Region-Language Alignment for Open-Vocabulary Dense Prediction

Pre-trained vision-language models (VLMs), such as CLIP, have demonstrated impressive zero-shot recognition capability, but still underperform in dense prediction tasks. Self-distillation recently is emerging as a promising approach for fine-tuning VLMs to better adapt to local regions without requiring extensive annotations. However, previous state-of-the-art approaches often suffer from significant `foreground bias', where models tend to wrongly identify background regions as foreground objects. To alleviate this issue, we propose DenseVLM, a framework designed to learn unbiased region-language alignment from powerful pre-trained VLM representations. To alleviate this issue, we propose DenseVLM, a framework designed to learn unbiased region-language alignment from powerful pre-trained VLM representations. DenseVLM leverages the pre-trained VLM to retrieve categories for unlabeled regions and then decouples the interference between foreground and background features. We show that DenseVLM can directly replace the original VLM in open-vocabulary object detection and image segmentation methods, leading to notable performance improvements. Furthermore, it exhibits promising zero-shot scalability when training on more extensive and diverse datasets. Our code is available at https://github.com/HVision-NKU/DenseVLM.

==> figs/Framework.tex <==
\begin{figure*}[t]
    \centering
    % \small
    \begin{overpic}[width=0.99\textwidth]{images/framework.pdf}
    \put(33.5,30.8){$\mathcal{F}^1_{P}$}
    \put(40,30.8){$\mathcal{F}^2_{P}$}
    \put(46.5,30.8){$\mathcal{F}^k_{P}$}
    \put(53.5,30.8){$\mathcal{F}^{m \times n}_{P}$}

    \put(68.5,30.8){$\mathcal{F}^1_{L}$}
    \put(75.7,30.8){$\mathcal{F}^2_{L}$}
    \put(83,30.8){$\mathcal{F}^k_{L}$}
    \put(92.5,30.8){$\mathcal{F}^{m \times n}_{L}$}
  
    \put(39.6,20.9){$\mathcal{T}^1_{P}$}
    \put(44.3,20.9){$\mathcal{T}^2_{P}$}
    \put(51.0,20.9){$\mathcal{T}^D_{P}$}

    \put(37,11){$\mathcal{F}^u_{P}$}
    \put(41.7,11){$\mathcal{T}^u_{P}$}

    \put(49.7,11){$\mathcal{F}^v_{P}$}
    \put(54.5,11){$\mathcal{T}^v_{P}$}

    \put(61.3,33){{$k$}}
    \put(5.5,4.5){{$\{c^1, \dots, c^D\}$}}

    \put(60,7){{$(k, c^k)$}}

    \put(74.5,22){$\mathcal{F}^u_{L}$}
    \put(87.5,22){$\mathcal{F}^v_{L}$}

    \put(70,11.5){$\mathcal{T}^1_{L}$}
    \put(77,11.5){$\mathcal{T}^u_{L}$}

    \put(85,11.5){$\mathcal{T}^1_{L}$}
    \put(92,11.5){$\mathcal{T}^v_{L}$}
    
    \end{overpic}
    \vspace{-5pt}
    \caption{{Overview of \methodname{}.}
    % 
    For clarity, this diagram omits the dense visual and text features extracted by the training VLM (L-VLM), 
    which are similar to those extracted by a more powerful VLM (P-VLM).
    % 
    % By leveraging the powerful VLM, \methodname{} retrieves categories for unlabeled regions and 
    % identifies foreground and background regions.
    \methodname{} leverages the powerful VLM to \textbf{retrieve} categories for unlabeled regions 
    and distinguish between foreground and background.
    % 
    During VLM training, \methodname{} \textbf{decouples} interference between features of foreground and background regions, 
    \textbf{aligning} each region with its corresponding text embeddings.
    }
    \label{fig: framework}
    \vspace{-5pt}
  \end{figure*}

==> figs/Framework_old.tex <==
\begin{figure*}[t]
    \centering
    % \small
    \begin{overpic}[width=0.99\textwidth]{images/Framework_old.pdf}
    % \put(33.5,30.8){$\mathcal{F}^1_{P}$}
    % \put(40,30.8){$\mathcal{F}^2_{P}$}
    % \put(46.5,30.8){$\mathcal{F}^k_{P}$}
    % \put(53.5,30.8){$\mathcal{F}^{m \times n}_{P}$}

    % \put(68.5,30.8){$\mathcal{F}^1_{L}$}
    % \put(75.7,30.8){$\mathcal{F}^2_{L}$}
    % \put(83,30.8){$\mathcal{F}^k_{L}$}
    % \put(92.5,30.8){$\mathcal{F}^{m \times n}_{L}$}
  
    \put(24.5,20.3){$\mathcal{T}^1_{P}$}
    \put(28.6,20.3){$\mathcal{T}^2_{P}$}
    \put(35.0,20.3){$\mathcal{T}^D_{P}$}

    \put(43,12.5){$\mathcal{F}^u_{P}$}
    \put(43,9.5){$\mathcal{T}^u_{P}$}

    \put(52.5,12.5){$\mathcal{F}^v_{P}$}
    \put(52.5,9.5){$\mathcal{T}^v_{P}$}

    \put(45.8,28.5){{$k$}}
    \put(69.3,28.5){{$k$}}
    \put(3,4.5){{$\{c^1, \dots, c^D\}$}}

    \put(59,8){{$(k, c^k)$}}

    \put(84.3,28.6){$\mathcal{T}^1_{L}$}
    \put(88.3,28.6){$\mathcal{T}^2_{L}$}
    \put(94.7,28.6){$\mathcal{T}^D_{L}$}

    \put(74,18.8){$\mathcal{F}^u_{L}$}
    \put(88.5,18.8){$\mathcal{F}^v_{L}$}

    \put(69,6){$\mathcal{T}^1_{L}$}
    \put(75.5,6){$\mathcal{T}^u_{L}$}

    \put(84,6){$\mathcal{T}^1_{L}$}
    \put(90.3,6){$\mathcal{T}^v_{L}$}

    \end{overpic}
    \vspace{-10pt}
    \caption{{Overview of \methodname{}.}
    % 
    For clarity, this diagram omits the dense visual and text features extracted by the training VLM (L-VLM), 
    which are similar to those extracted by the powerful VLM (P-VLM).
    % 
    % By leveraging the powerful VLM, \methodname{} retrieves categories for unlabeled regions and 
    % identifies foreground and background regions.
    \methodname{} leverages the powerful VLM to \textbf{retrieve} categories for unlabeled regions 
    and distinguish between foreground and background.
    % 
    During VLM training, \methodname{} \textbf{decouples} interference between features of foreground and background regions, 
    \textbf{aligning} each region with its corresponding text embeddings.
    }
    \vspace{-5pt}
    \label{fig: framework}
  \end{figure*}

==> tables/9_generate_labels.tex <==
\begin{table}[t]
  \centering
  \tablestyle{6.pt}{1.0}
  \centering
  \small
  \begin{tabular}{l cc cc cc}
  \toprule
    &\multicolumn{2}{c}{\textbf{Boxes}}  &\multicolumn{2}{c}{\textbf{Masks-T}}&\multicolumn{2}{c}{\textbf{Masks-S}} \\
  \multirow{1}{*}{Categories} &Top1&Top5&Top1&Top5& Top1&Top5\\
  \midrule
  133 (80)& 71.1& 88.5& 68.7& 83.0& 44.7& 75.2 \\
  171 (80)& 72.3& 89.8& 69.4& 85.8& 44.2& 76.0 \\
  273 (160)& 72.3& 89.9& 70.1& 84.4& 44.9& 76.4 \\
  316 (204)& \textbf{73.4}& \textbf{90.5}& \textbf{71.0}& \textbf{84.8}& \textbf{45.6}& \textbf{77.8}\\
  \bottomrule
  \end{tabular}
\vspace{-5pt}
\caption{
{Ablation study on category sets}.
% 
The numbers in parentheses denote the number of foreground thing classes.
% 
}
\label{tab: categories}
\vspace{-10pt}
\end{table}

